ENO-Based High-Order Data-Bounded and Constrained Positivity-Preserving Interpolation

A number of key scientific computing applications that are based upon tensor-product grid constructions, such as numerical weather prediction (NWP) and combustion simulations, require property-preserving interpolation. Essentially non-oscillatory (ENO) interpolation is a classic example of such interpolation schemes. In the aforementioned application areas, property preservation often manifests itself as a requirement for either data boundedness or positivity preservation. For example, in NWP, one may have to interpolate between the grid on which the dynamics is calculated to a grid on which the physics is calculated (and back). Interpolating density or other key physical quantities without accounting for property preservation may lead to negative values that are nonphysical and result in inaccurate representations and/or interpretations of the physical data. Property-preserving interpolation is straightforward when used in the context of low-order numerical simulation methods. High-order property-preserving interpolation is, however, nontrivial, especially in the case where the interpolation points are not equispaced. In this paper, we demonstrate that it is possible to construct high-order interpolation methods that ensure either data boundedness or constrained positivity preservation. A novel feature of the algorithm is that the positivity-preserving interpolant is constrained; that is, the amount by which it exceeds the data values may be strictly controlled. The algorithm we have developed comes with theoretical estimates that provide sufficient conditions for data boundedness and constrained positivity preservation. We demonstrate the application of our algorithm on a collection of 1D and 2D numerical examples, and show that in all cases property preservation is respected.

==> out <==
Warning: MATLAB has disabled some advanced graphics rendering features by switching to software OpenGL. For more information, click here. 
Comparing DBI and PPI against PCHIP 
 ------- fun = 1  -------- 
17 	 & 7.15E-03   & 0.00   & 1.05E-02   & 0.00   & 1.67E-02   & 0.00   && 4.75E-03   & 0.00   & 7.90E-03   & 0.00   & 7.92E-03   & 0.00   \\ 
33 	 & 1.91E-03   & 1.99   & 1.14E-03   & 3.33   & 1.61E-03   & 3.53   && 1.30E-03   & 1.96   & 2.44E-03   & 1.77   & 2.44E-03   & 1.77   \\ 
65 	 & 3.70E-04   & 2.42   & 9.70E-05   & 3.64   & 1.17E-04   & 3.87   && 2.86E-04   & 2.23   & 2.40E-04   & 3.42   & 2.40E-04   & 3.42   \\ 
129 	 & 6.79E-05   & 2.47   & 6.81E-06   & 3.88   & 7.59E-06   & 3.99   && 5.81E-05   & 2.32   & 1.29E-05   & 4.27   & 1.29E-05   & 4.27   \\ 
257 	 & 1.22E-05   & 2.49   & 4.51E-07   & 3.94   & 4.79E-07   & 4.01   && 1.15E-05   & 2.35   & 1.26E-06   & 3.37   & 1.26E-06   & 3.37   \\ 
 ------- fun = 2  -------- 
17 	 & 2.02E-02   & 0.00   & 1.97E-02   & 0.00   & 1.97E-02   & 0.00   && 3.65E-03   & 0.00   & 5.38E-03   & 0.00   & 5.38E-03   & 0.00   \\ 
33 	 & 3.38E-03   & 2.70   & 3.53E-03   & 2.59   & 3.53E-03   & 2.59   && 1.45E-03   & 1.39   & 1.55E-03   & 1.88   & 1.55E-03   & 1.88   \\ 
65 	 & 3.59E-04   & 3.31   & 6.70E-04   & 2.45   & 6.77E-04   & 2.44   && 4.07E-04   & 1.87   & 6.40E-04   & 1.30   & 6.42E-04   & 1.30   \\ 
129 	 & 4.21E-05   & 3.13   & 5.31E-05   & 3.70   & 5.31E-05   & 3.71   && 8.85E-05   & 2.23   & 1.00E-04   & 2.70   & 1.00E-04   & 2.71   \\ 
257 	 & 5.12E-06   & 3.06   & 3.54E-06   & 3.93   & 3.54E-06   & 3.93   && 1.38E-05   & 2.70   & 1.14E-05   & 3.16   & 1.14E-05   & 3.16   \\ 
 ------- Function fun = 1  -------- 
 ---- Polynomial degree d = 1  ---- 
17 	  & 2.16E-02   & 0.00   & 2.16E-02   & 0.00   && 1.69E-02   & 0.00   & 1.69E-02   & 0.00   \\ 
33 	  & 6.02E-03   & 1.92   & 6.02E-03   & 1.92   && 5.84E-03   & 1.60   & 5.84E-03   & 1.60   \\ 
65 	  & 1.52E-03   & 2.03   & 1.52E-03   & 2.03   && 1.66E-03   & 1.86   & 1.66E-03   & 1.86   \\ 
129 	  & 3.82E-04   & 2.02   & 3.82E-04   & 2.02   && 5.80E-04   & 1.53   & 5.80E-04   & 1.53   \\ 
257 	  & 9.56E-05   & 2.01   & 9.56E-05   & 2.01   && 1.52E-04   & 1.94   & 1.52E-04   & 1.94   \\ 
 ---- Polynomial degree d = 4  ---- 
17 	  & 8.34E-03   & 0.00   & 7.02E-03   & 0.00   && 6.54E-03   & 0.00   & 6.54E-03   & 0.00   \\ 
33 	  & 6.72E-04   & 3.80   & 5.91E-04   & 3.73   && 7.63E-04   & 3.24   & 7.62E-04   & 3.24   \\ 
65 	  & 4.55E-05   & 3.97   & 2.39E-05   & 4.73   && 5.30E-05   & 3.93   & 5.29E-05   & 3.94   \\ 
129 	  & 2.68E-06   & 4.13   & 8.00E-07   & 4.95   && 3.44E-06   & 3.99   & 3.44E-06   & 3.99   \\ 
257 	  & 8.63E-08   & 4.99   & 2.55E-08   & 5.00   && 8.88E-08   & 5.31   & 8.87E-08   & 5.31   \\ 
 ---- Polynomial degree d = 8  ---- 
17 	  & 4.61E-03   & 0.00   & 3.11E-03   & 0.00   && 5.61E-03   & 0.00   & 5.60E-03   & 0.00   \\ 
33 	  & 5.44E-04   & 3.22   & 1.51E-04   & 4.56   && 1.76E-04   & 5.22   & 1.76E-04   & 5.22   \\ 
65 	  & 4.01E-05   & 3.85   & 1.05E-06   & 7.33   && 3.26E-06   & 5.89   & 3.01E-06   & 6.00   \\ 
129 	  & 2.56E-06   & 4.01   & 3.10E-09   & 8.50   && 5.76E-08   & 5.89   & 8.82E-09   & 8.51   \\ 
257 	  & 8.24E-08   & 4.99   & 6.80E-12   & 8.88   && 3.51E-09   & 4.06   & 3.96E-11   & 7.84   \\ 
 ---- Polynomial degree d = 16  ---- 
17 	  & 4.64E-03   & 0.00   & 3.80E-03   & 0.00   && 6.52E-03   & 0.00   & 6.52E-03   & 0.00   \\ 
33 	  & 5.34E-04   & 3.26   & 4.85E-05   & 6.58   && 1.18E-04   & 6.05   & 1.17E-04   & 6.06   \\ 
65 	  & 4.01E-05   & 3.82   & 5.92E-08   & 9.89   && 1.25E-06   & 6.71   & 9.40E-08   & 10.51   \\ 
129 	  & 2.56E-06   & 4.01   & 4.21E-12   & 13.94   && 5.70E-08   & 4.50   & 1.02E-11   & 13.32   \\ 
257 	  & 8.24E-08   & 4.99   & 2.19E-16   & 14.31   && 3.51E-09   & 4.04   & 4.99E-16   & 14.39   \\ 
 ------- Function fun = 2  -------- 
 ---- Polynomial degree d = 1  ---- 
17 	  & 2.89E-02   & 0.00   & 2.89E-02   & 0.00   && 8.58E-03   & 0.00   & 8.58E-03   & 0.00   \\ 
33 	  & 7.69E-03   & 1.99   & 7.69E-03   & 1.99   && 5.24E-03   & 0.74   & 5.24E-03   & 0.74   \\ 
65 	  & 1.80E-03   & 2.14   & 1.80E-03   & 2.14   && 2.20E-03   & 1.28   & 2.20E-03   & 1.28   \\ 
129 	  & 4.58E-04   & 2.00   & 4.58E-04   & 2.00   && 8.08E-04   & 1.47   & 8.08E-04   & 1.47   \\ 
257 	  & 1.15E-04   & 2.00   & 1.15E-04   & 2.00   && 2.01E-04   & 2.01   & 2.01E-04   & 2.01   \\ 
 ---- Polynomial degree d = 4  ---- 
17 	  & 2.23E-02   & 0.00   & 2.23E-02   & 0.00   && 5.24E-03   & 0.00   & 5.24E-03   & 0.00   \\ 
33 	  & 4.09E-03   & 2.56   & 4.09E-03   & 2.56   && 1.10E-03   & 2.36   & 1.10E-03   & 2.36   \\ 
65 	  & 3.05E-04   & 3.83   & 3.05E-04   & 3.83   && 3.06E-04   & 1.88   & 3.07E-04   & 1.88   \\ 
129 	  & 1.35E-05   & 4.55   & 1.35E-05   & 4.55   && 3.32E-05   & 3.24   & 3.32E-05   & 3.24   \\ 
257 	  & 4.71E-07   & 4.87   & 4.71E-07   & 4.87   && 1.17E-06   & 4.85   & 1.17E-06   & 4.85   \\ 
 ---- Polynomial degree d = 8  ---- 
17 	  & 2.08E-02   & 0.00   & 2.08E-02   & 0.00   && 4.87E-03   & 0.00   & 4.87E-03   & 0.00   \\ 
33 	  & 3.36E-03   & 2.75   & 3.36E-03   & 2.75   && 8.71E-04   & 2.59   & 8.28E-04   & 2.67   \\ 
65 	  & 1.38E-04   & 4.70   & 1.38E-04   & 4.70   && 7.57E-05   & 3.60   & 7.17E-05   & 3.61   \\ 
129 	  & 1.22E-06   & 6.90   & 1.22E-06   & 6.90   && 2.17E-06   & 5.19   & 2.17E-06   & 5.11   \\ 
257 	  & 4.44E-09   & 8.15   & 4.44E-09   & 8.15   && 1.95E-08   & 6.83   & 1.95E-08   & 6.83   \\ 
 ---- Polynomial degree d = 16  ---- 
17 	  & 2.00E-02   & 0.00   & 2.00E-02   & 0.00   && 4.83E-03   & 0.00   & 4.83E-03   & 0.00   \\ 
33 	  & 2.93E-03   & 2.90   & 2.93E-03   & 2.90   && 7.38E-04   & 2.83   & 6.88E-04   & 2.94   \\ 
65 	  & 9.17E-05   & 5.11   & 9.17E-05   & 5.11   && 7.60E-05   & 3.35   & 7.27E-05   & 3.31   \\ 
129 	  & 1.70E-07   & 9.17   & 1.70E-07   & 9.17   && 2.88E-07   & 8.14   & 2.88E-07   & 8.07   \\ 
257 	  & 2.64E-11   & 12.73   & 2.64E-11   & 12.73   && 5.39E-11   & 12.45   & 5.39E-11   & 12.45   \\ 
 ------- Function fun = 1  -------- 
 ---- Polynomial degree d = 1  ---- 
16 	 & 2.81E-02   & 0.00   & 2.81E-02   & 0.00 \\  
32 	 & 6.41E-03   & 2.13   & 6.41E-03   & 2.13 \\  
64 	 & 1.57E-03   & 2.03   & 1.57E-03   & 2.03 \\  
128 	 & 3.88E-04   & 2.02   & 3.88E-04   & 2.02 \\  
256 	 & 9.63E-05   & 2.01   & 9.63E-05   & 2.01 \\  
 ---- Polynomial degree d = 4  ---- 
16 	 & 2.81E-02   & 0.00   & 1.37E-02   & 0.00 \\  
32 	 & 4.72E-03   & 2.57   & 6.85E-04   & 4.32 \\  
64 	 & 8.14E-04   & 2.54   & 2.57E-05   & 4.73 \\  
128 	 & 1.42E-04   & 2.52   & 8.32E-07   & 4.95 \\  
256 	 & 2.49E-05   & 2.51   & 2.60E-08   & 5.00 \\  
 ---- Polynomial degree d = 8  ---- 
16 	 & 2.74E-02   & 0.00   & 1.07E-02   & 0.00 \\  
32 	 & 4.69E-03   & 2.55   & 2.06E-04   & 5.70 \\  
64 	 & 8.14E-04   & 2.53   & 1.19E-06   & 7.43 \\  
128 	 & 1.42E-04   & 2.52   & 3.32E-09   & 8.49 \\  
256 	 & 2.49E-05   & 2.51   & 7.04E-12   & 8.88 \\  
 ---- Polynomial degree d = 16  ---- 
16 	 & 2.75E-02   & 0.00   & 1.01E-02   & 0.00 \\  
32 	 & 4.69E-03   & 2.55   & 1.43E-04   & 6.14 \\  
64 	 & 8.14E-04   & 2.53   & 7.18E-08   & 10.96 \\  
128 	 & 1.42E-04   & 2.52   & 4.74E-12   & 13.89 \\  
256 	 & 2.49E-05   & 2.51   & 2.81E-16   & 14.04 \\  
>> 


==> result-long-table.tex <==
\section{Numerical Experiments}
\label{sec:results}

------- Function fun = 1  -------- 
 ---- Polynomial degree d = 4  ---- 
17 	 7.153219e-03 	 0 	 8.338289e-03 	 0 	 7.022246e-03 	 0 	 17 	 1.021031e-02 	 0 	 8.631043e-03 	 0 	 8.386141e-03 	 0 
33 	 1.909142e-03 	 1.991437e+00 	 6.722050e-04 	 3.796279e+00 	 5.905622e-04 	 3.732527e+00 	 33 	 1.857245e-03 	 2.569454e+00 	 7.945207e-04 	 3.596265e+00 	 7.803241e-04 	 3.580050e+00 
65 	 3.698019e-04 	 2.421435e+00 	 4.554679e-05 	 3.970945e+00 	 2.386616e-05 	 4.733308e+00 	 65 	 3.679343e-04 	 2.388248e+00 	 4.771166e-05 	 4.149060e+00 	 4.636664e-05 	 4.164646e+00 
129 	 6.786452e-05 	 2.473580e+00 	 2.681504e-06 	 4.132271e+00 	 8.004920e-07 	 4.953116e+00 	 129 	 7.200433e-05 	 2.379805e+00 	 1.489516e-06 	 5.057772e+00 	 1.267424e-06 	 5.251622e+00 
257 	 1.222110e-05 	 2.487218e+00 	 8.626651e-08 	 4.986033e+00 	 2.547612e-08 	 5.001692e+00 	 257 	 1.522212e-05 	 2.254546e+00 	 4.680091e-08 	 5.020291e+00 	 3.949535e-08 	 5.032267e+00 
 ---- Polynomial degree d = 8  ---- 
17 	 7.153219e-03 	 0 	 4.606019e-03 	 0 	 3.354274e-03 	 0 	 17 	 4.753337e-03 	 0 	 5.606832e-03 	 0 	 6.192262e-03 	 0 
33 	 1.909142e-03 	 1.991437e+00 	 5.442048e-04 	 3.219979e+00 	 1.514660e-04 	 4.670068e+00 	 33 	 1.295061e-03 	 1.960350e+00 	 1.763666e-04 	 5.215146e+00 	 1.757587e-04 	 5.370081e+00 
65 	 3.698019e-04 	 2.421435e+00 	 4.014371e-05 	 3.845608e+00 	 1.051356e-06 	 7.332098e+00 	 65 	 2.859827e-04 	 2.228098e+00 	 3.259368e-06 	 5.887522e+00 	 3.013481e-06 	 5.998138e+00 
129 	 6.786452e-05 	 2.473580e+00 	 2.563353e-06 	 4.013786e+00 	 3.102637e-09 	 8.499227e+00 	 129 	 5.814046e-05 	 2.324206e+00 	 5.763441e-08 	 5.887103e+00 	 8.815598e-09 	 8.511985e+00 
257 	 1.222110e-05 	 2.487218e+00 	 8.242271e-08 	 4.986786e+00 	 6.795344e-12 	 8.884510e+00 	 257 	 1.151771e-05 	 2.348848e+00 	 3.512224e-09 	 4.059216e+00 	 3.962279e-11 	 7.841518e+00 
 ---- Polynomial degree d = 16  ---- 
17 	 7.153219e-03 	 0 	 4.637155e-03 	 0 	 1.111673e-01 	 0 	 17 	 7.803600e-03 	 0 	 9.185328e-03 	 0 	 2.196900e-02 	 0 
33 	 1.909142e-03 	 1.991437e+00 	 5.344161e-04 	 3.257501e+00 	 4.846943e-05 	 1.166580e+01 	 33 	 6.149435e-04 	 3.830593e+00 	 5.865194e-05 	 7.619156e+00 	 5.862725e-05 	 8.934479e+00 
65 	 3.698019e-04 	 2.421435e+00 	 4.013502e-05 	 3.819152e+00 	 5.922046e-08 	 9.894708e+00 	 65 	 1.611768e-04 	 1.975318e+00 	 1.407266e-07 	 8.899156e+00 	 1.166760e-07 	 9.175011e+00 
129 	 6.786452e-05 	 2.473580e+00 	 2.563351e-06 	 4.013471e+00 	 4.207419e-12 	 1.393613e+01 	 129 	 3.775379e-05 	 2.117542e+00 	 3.517458e-09 	 5.382178e+00 	 4.442502e-11 	 1.148682e+01 
257 	 1.222110e-05 	 2.487218e+00 	 8.242271e-08 	 4.986785e+00 	 2.193762e-16 	 1.430740e+01 	 257 	 8.101652e-06 	 2.232843e+00 	 1.559620e-10 	 4.520595e+00 	 2.969642e-15 	 1.394694e+01 
 ------- Function fun = 2  -------- 
 ---- Polynomial degree d = 4  ---- 
17 	 2.023486e-02 	 0 	 2.234591e-02 	 0 	 2.311749e-02 	 0 	 17 	 8.598583e-03 	 0 	 1.255664e-02 	 0 	 2.148116e-02 	 0 
33 	 3.377348e-03 	 2.699129e+00 	 4.094897e-03 	 2.558294e+00 	 4.475200e-03 	 2.475581e+00 	 33 	 2.503690e-03 	 1.860157e+00 	 3.109658e-03 	 2.104249e+00 	 4.692973e-03 	 2.293266e+00 
65 	 3.589393e-04 	 3.306918e+00 	 3.046392e-04 	 3.833082e+00 	 3.046392e-04 	 3.964093e+00 	 65 	 6.357460e-04 	 2.022073e+00 	 3.417871e-04 	 3.257333e+00 	 3.720557e-04 	 3.739274e+00 
129 	 4.205611e-05 	 3.128202e+00 	 1.347978e-05 	 4.548910e+00 	 1.347978e-05 	 4.548910e+00 	 129 	 1.017910e-04 	 2.672616e+00 	 1.548728e-05 	 4.514233e+00 	 1.548728e-05 	 4.638033e+00 
257 	 5.118935e-06 	 3.055519e+00 	 4.710576e-07 	 4.866013e+00 	 4.710576e-07 	 4.866013e+00 	 257 	 1.834996e-05 	 2.485687e+00 	 6.287151e-07 	 4.648579e+00 	 6.287151e-07 	 4.648579e+00 
 ---- Polynomial degree d = 8  ---- 
17 	 2.023486e-02 	 0 	 2.083789e-02 	 0 	 2.148785e-02 	 0 	 17 	 3.649025e-03 	 0 	 4.865633e-03 	 0 	 2.729587e-02 	 0 
33 	 3.377348e-03 	 2.699129e+00 	 3.356153e-03 	 2.752893e+00 	 3.653528e-03 	 2.671205e+00 	 33 	 1.450648e-03 	 1.390710e+00 	 8.707063e-04 	 2.594094e+00 	 3.394995e-03 	 3.142546e+00 
65 	 3.589393e-04 	 3.306918e+00 	 1.383931e-04 	 4.703566e+00 	 1.383931e-04 	 4.828807e+00 	 65 	 4.071188e-04 	 1.874463e+00 	 7.572240e-05 	 3.602749e+00 	 1.221982e-04 	 4.904135e+00 
129 	 4.205611e-05 	 3.128202e+00 	 1.223897e-06 	 6.897993e+00 	 1.223897e-06 	 6.897993e+00 	 129 	 8.853271e-05 	 2.225966e+00 	 2.165462e-06 	 5.185746e+00 	 2.165462e-06 	 5.883955e+00 
257 	 5.118935e-06 	 3.055519e+00 	 4.444264e-09 	 8.150990e+00 	 4.444264e-09 	 8.150990e+00 	 257 	 1.377123e-05 	 2.699678e+00 	 1.954223e-08 	 6.830203e+00 	 1.954223e-08 	 6.830203e+00 
 ---- Polynomial degree d = 16  ---- 
17 	 2.023486e-02 	 0 	 1.999322e-02 	 0 	 3.845265e-02 	 0 	 17 	 3.883998e-02 	 0 	 3.766154e-02 	 0 	 3.706627e-02 	 0 
33 	 3.377348e-03 	 2.699129e+00 	 2.930038e-03 	 2.895212e+00 	 3.167959e-03 	 3.763549e+00 	 33 	 6.196593e-04 	 6.238613e+00 	 2.534743e-04 	 7.539840e+00 	 7.572617e-03 	 2.394365e+00 
65 	 3.589393e-04 	 3.306918e+00 	 9.167009e-05 	 5.110899e+00 	 9.167068e-05 	 5.226060e+00 	 65 	 1.929874e-04 	 1.720873e+00 	 1.373614e-05 	 4.300516e+00 	 7.463455e-05 	 6.814912e+00 
129 	 4.205611e-05 	 3.128202e+00 	 1.703397e-07 	 9.174097e+00 	 1.703397e-07 	 9.174107e+00 	 129 	 5.300640e-05 	 1.885271e+00 	 2.192745e-07 	 6.036343e+00 	 2.192745e-07 	 8.505720e+00 
257 	 5.118935e-06 	 3.055519e+00 	 2.642730e-11 	 1.272539e+01 	 2.642730e-11 	 1.272539e+01 	 257 	 1.139476e-05 	 2.230291e+00 	 1.560666e-10 	 1.051527e+01 	 1.560666e-10 	 1.051527e+01 
>> 



  In this section we present both 1D and 2D numerical experiments which demonstrate the properties of our proposed methods.
  These experimental studies use the PCHIP, DBI and PPI methods.
  The test functions used here are taken from test problem XX and XX in \cite{arkivtajo}.
  A full suite test problem has been undertaken by the authors in \cite{arkivtajo}. 
  In that study, nine test problems are used with both uniform and nonuniform (LGL) meshes.
  Herein we only summarize those results by presenting two representative problems with LGL meshes being shown.
 
  \subsection{1D Example: Runge Function}
  \label{subsec:1d_runge}
    This example uses the Runge ~\cite{doi:10.1080/00029890.1987.12000642} function defined as follows:
    \begin{equation}\label{eq:1d_runge}
      f_{1}(x) = \frac{1}{1+25x^2}, \quad x\in [-1,1].
    \end{equation}

    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c c  c  c c  c  c c}
        \hline
        $N_{i}$   & PCHIP     & Rate    && DBI      & Rate     &&  PPI      & Rate  \\
        \hline
          $13 $   & 8.70E-3   & -- 	&& 2.06E-2  & --       && 3.79E-2   & --    \\ 	 
          $25 $   & 3.57E-3   & 1.34 	&& 3.13E-3  & 2.84     && 4.46E-3   & 3.23  \\	 
          $49 $   & 7.39E-4   & 2.32 	&& 3.13E-4  & 3.40     && 3.55E-4   & 3.74  \\	 
          $97 $   & 1.38E-4   & 2.45 	&& 2.09E-5  & 3.95     && 2.37E-5   & 3.94  \\	 
          $193$   & 2.49E-5   & 2.49 	&& 1.40E-6  & 3.93     && 1.51E-6   & 4.00  \\	 
        \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the PCHIP method to approximate the function $f_{1}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               The interval $[-1,1]$ is divided into $(N_{i}-1) / 3$ elements and $4$ uniform points are used in each element.}
      \label{tab:f1_PCHIP}
    \end{table}
    %
    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c  c  c  c  c}
        \hline
        $N_{i}$   & \multicolumn{2}{c}{DBI} && \multicolumn{2}{c}{PPI}   \\
        \hline
                  & $L^{2}$-error & Rate     && $L^{2}$-error & Rate     \\ 
        \hline
                  & \multicolumn{5}{c}{$\mathcal{P}_{1}$}               \\
        \hline
          $17 $	  & 2.16E-2   & -- 	&& 2.16E-2     & -- 	\\ 
          $33 $	  & 6.02E-3   & 1.92 	&& 6.02E-3     & 1.92 	\\ 
          $65 $	  & 1.52E-3   & 2.03 	&& 1.52E-3     & 2.03 	\\ 
          $129$   & 3.82E-4   & 2.02 	&& 3.82E-4     & 2.02 	\\ 
          $257$   & 9.56E-5   & 2.01 	&& 9.56E-5     & 2.01 	\\        
        \hline
                  & \multicolumn{5}{c}{$\mathcal{P}_{4}$}               \\
        \hline
          $17 $	  & 8.34E-3 & 0 	 && 7.02E-3 	 & 0 	 \\
          $33 $	  & 6.72E-4 & 3.80	 && 5.91E-4 	 & 3.73	 \\
          $65 $	  & 4.55E-5 & 3.97	 && 2.39E-5 	 & 4.73	 \\
          $129$   & 2.68E-6 & 4.13	 && 8.00E-7 	 & 4.95	 \\
          $257$   & 8.63E-8 & 4.99	 && 2.55E-8 	 & 5.00	 \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{8}$}               \\
        \hline
          $17 $	  & 4.61E-3 	 & 0 	 && 3.35E-3 	 & 0 	 \\
          $33 $	  & 5.44E-4 	 & 3.22	 && 1.51E-4 	 & 4.67	 \\
          $65 $	  & 4.01E-5 	 & 3.85	 && 1.05E-6 	 & 7.33	 \\
          $129$   & 2.56E-6 	 & 4.01	 && 3.10E-9 	 & 8.50	 \\
          $257$   & 8.24E-8 	 & 4.99	 && 6.80E-12 	 & 8.88	 \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{16}$}               \\
        \hline
          $17 $	  & 4.64E-3 	 & 0 	 && 1.11E-1 	 & 0 	 \\
          $33 $	  & 5.34E-4 	 & 3.26	 && 4.85E-5 	 & 11.67 \\
          $65 $	  & 4.01E-5 	 & 3.82	 && 5.92E-8 	 & 9.894 \\
          $129$	  & 2.56E-6 	 & 4.01	 && 4.21E-12 	 & 13.94 \\
          $257$   & 8.24E-8 	 & 4.99	 && 2.19E-16 	 & 14.31 \\
     \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the DBI and PPI methods to approximate the function $f_{1}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               $\mathcal{P}_{j}$ represents the use of polynomials of degree $ \leq j$, with $j$ being the target degree for each of interval.
               The interval $[-1,1]$ is divided into $(N_{i}-1) / j$ elements and $j+1$ uniform points are used in each element.}
      \label{tab:f1_DBI_PPI_LGL}
    \end{table}
    %% 
    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c c  c  c c  c  c c}
        \hline
        $N_{i}$   & PCHIP     & Rate    && DBI      & Rate     &&  PPI      & Rate  \\
        \hline
          $17 $	  & 1.81E-2   & -- 	&& 1.97E-2  & --       && 3.17E-2   & --    \\ 
          $33 $	  & 4.55E-3   & 2.08 	&& 3.44E-3  & 2.63     && 3.79E-3   & 3.20  \\
          $65 $	  & 7.06E-4   & 2.75 	&& 4.25E-4  & 3.08     && 4.32E-4   & 3.20  \\
          $129$	  & 1.40E-4   & 2.36 	&& 2.92E-5  & 3.91     && 3.01E-5   & 3.89  \\
          $257$	  & 3.11E-5   & 2.18 	&& 1.87E-6  & 3.99     && 1.91E-6   & 4.00  \\
        \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the PCHIP method to approximate the function $f_{1}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               The interval $[-1,1]$ is divided into $(N_{i}-1) / 3$ elements and $4$ uniform points are used in each element.}
      \label{tab:f1_PCHIP}
    \end{table}
    %% 
    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c  c  c  c  c}
        \hline
        $N_{i}$     & \multicolumn{2}{c}{DBI} && \multicolumn{2}{c}{PPI}   \\
        \hline
                    & $L^{2}$-error & Rate     && $L^{2}$-error & Rate     \\ 
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{1}$}               \\
        \hline
          $17 $	    & 1.91E-2 	& -- 	       && 1.91E-2 	& --       \\	
          $33 $	    & 5.55E-3 	& 1.86 	       && 5.55E-3 	& 1.86 	   \\
          $65 $	    & 2.05E-3 	& 1.47 	       && 2.05E-3 	& 1.47 	   \\
          $129$     & 5.40E-4 	& 1.95 	       && 5.40E-4 	& 1.95 	   \\
          $257$     & 1.35E-4 	& 2.01 	       && 1.35E-4 	& 2.01 	   \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{4}$}               \\
        \hline
     $17 $	 & 8.63E-3 	 & 0 	         && 8.39E-3 	 & 0     \\ 
     $33 $	 & 7.95E-4 	 & 3.60 	 && 7.80E-4 	 & 3.58  \\
     $65 $	 & 4.77E-5 	 & 4.15 	 && 4.64E-5 	 & 4.16  \\
     $129$ 	 & 1.49E-6 	 & 5.06 	 && 1.27E-6 	 & 5.25  \\
     $257$ 	 & 4.68E-8 	 & 5.02 	 && 3.95E-8 	 & 5.03  \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{8}$}               \\
        \hline
     $17 $	 & 5.60E-3 	 & 0 	         && 6.19E-3 	 & 0     \\
     $33 $	 & 1.76E-4 	 & 5.22 	 && 1.76E-4 	 & 5.37  \\
     $65 $	 & 3.26E-6 	 & 5.89 	 && 3.01E-6 	 & 6.00  \\
     $129$ 	 & 5.76E-8 	 & 5.89 	 && 8.82E-9 	 & 8.51  \\
     $257$ 	 & 3.51E-9 	 & 4.06 	 && 3.96E-11 	 & 7.84  \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{16}$}               \\
        \hline
     $17 $	 & 9.19E-3 	 & 0 	         && 2.20E-2 	 & 0     \\
     $33 $	 & 5.87E-5 	 & 7.61 	 && 5.86E-5 	 & 8.93  \\
     $65 $	 & 1.41E-7 	 & 8.90 	 && 1.17E-7 	 & 9.17  \\
     $129$ 	 & 3.52E-9 	 & 5.38 	 && 4.44E-11 	 & 11.49 \\
     $257$ 	 & 1.56E-10 	 & 4.52 	 && 2.97E-15 	 & 13.95 \\
    \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the DBI and PPI methods to approximate the function $f_{1}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               $\mathcal{P}_{j}$ represents the use of polynomials of degree $ \leq j$, with $j$ being the target degree for each of interval.
               The interval $[-1,1]$ is divided into $(N_{i}-1) / j$ elements and $j+1$ uniform points are used in each element.}
      \label{tab:f1_DBI_PPI_LGL}
    \end{table}
 



  \subsection{1D Example: Smoothed Heaviside Function}
  \label{subsec:1d_example}
  %%
    The first test case on which we test our new methods is an analytic approximation of the Heaviside function defined as
    \begin{equation}\label{eq:f2}
         f_{2}(x) = \frac{1}{1+ e^{-2kx}}, \quad k=100 \textrm{, and } x \in [-0.2,0.2].
    \end{equation}
    A polynomial approximation of $f_{1}(x)$ is challenging because of the large solution gradient around $x =0.$
    Attempts to use a global polynomial approximation for this function result in oscillations and negative values.

    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c c  c  c c  c  c c}
        \hline
        $N_{i}$   & PCHIP     & Rate    && DBI      & Rate      &&  PPI      & Rate  \\
        \hline
          $13 $	  & 3.26E-2   & -- 	&& 3.16E-2  & -- 	&& 3.42E-2   & --     \\ 	 
          $25 $	  & 7.95E-3   & 2.13 	&& 7.91E-3  & 2.09 	&& 1.05E-2   & 1.78   \\	 
          $49 $	  & 8.96E-4   & 3.22 	&& 1.08E-3  & 2.93 	&& 1.73E-3   & 2.66   \\	 
          $97 $	  & 1.02E-4   & 3.17 	&& 1.58E-4  & 2.81 	&& 1.58E-4   & 3.49   \\	 
          $193$   & 1.22E-5   & 3.08 	&& 1.10E-5  & 3.86 	&& 1.10E-5   & 3.86   \\	 
       \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the PCHIP method to approximate the function $f_{2}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               The interval $[-0.2,0.2]$ is divided into $(N_{i}-1) / 3$ elements and $4$ uniform points are used in each element.}
      \label{tab:f2_PCHIP}
    \end{table}
    %%%
    \begin{table}[H]
      \centering
      \begin{tabular}{ c| c  c  c  c  c}
        \hline
        $N_{i}$     & \multicolumn{2}{c}{DBI} && \multicolumn{2}{c}{PPI}   \\
        \hline
                    & $L^{2}$-error & Rate     && $L^{2}$-error & Rate     \\ 
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{1}$}               \\
        \hline
        $17$        & 2.89E-2 	    & -- 	&& 2.89E-2   & -- 	   \\
        $33$        & 7.69E-3 	    & 1.99 	&& 7.69E-3   & 1.99 	   \\
        $65$        & 1.80E-3 	    & 2.14 	&& 1.80E-3   & 2.14 	   \\
        $129$       & 4.58E-4 	    & 2.00 	&& 4.58E-4   & 2.00 	   \\
        $257$       & 1.15E-4 	    & 2.00 	&& 1.15E-4   & 2.00 	   \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{4}$}               \\
        \hline
          $17 $	 & 2.23E-2 	 & -- 	         && 2.31E-2 	 & -- 	  \\           
          $33 $	 & 4.09E-3 	 & 2.56 	 && 4.48E-3 	 & 2.48   \\           
          $65 $	 & 3.05E-4 	 & 3.83 	 && 3.05E-4 	 & 3.96   \\           
          $129$	 & 1.35E-5 	 & 4.55 	 && 1.35E-5 	 & 4.55   \\           
          $257$	 & 4.71E-7 	 & 4.87 	 && 4.71E-7 	 & 4.87   \\           
                 \hline
                             & \multicolumn{5}{c}{$\mathcal{P}_{8}$}      \\
                 \hline
          $17 $	 & 2.08E-2 	 & -- 	         && 2.15E-2 	 & --	  \\           
          $33 $	 & 3.36E-3 	 & 2.75 	 && 3.65E-3 	 & 2.67   \\           
          $65 $	 & 1.38E-4 	 & 4.70 	 && 1.38E-4 	 & 4.83   \\           
          $129$  & 1.22E-6 	 & 6.90 	 && 1.22E-6 	 & 6.90   \\           
          $257$  & 4.44E-9 	 & 8.15 	 && 4.44E-9 	 & 8.15   \\           
                \hline
                            & \multicolumn{5}{c}{$\mathcal{P}_{16}$}      \\
                \hline
          $17 $	 & 2.00E-2 	 & -- 	         && 3.85E-2 	 & --	  \\           
          $33 $	 & 2.93E-3 	 & 2.90 	 && 3.17E-3 	 & 3.76   \\           
          $65 $	 & 9.17E-5 	 & 5.11 	 && 9.17E-5 	 & 5.23   \\           
          $129$  & 1.70E-7 	 & 9.17 	 && 1.70E-7 	 & 9.17   \\           
          $257$  & 2.64E-11 	 & 12.73 	 && 2.64E-11 	 & 12.73  \\           
        \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the DBI and PPI methods to approximate the function $f_{1}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               $\mathcal{P}_{j}$ represents the use of polynomials of degree $ \leq j$, with $j$ being the target degree for each of interval.
               The interval $[-0.2,0.2]$ is divided into $(N_{i}-1) / j$ elements and $j+1$ LGL quadrature points are used in each element.}
      \label{tab:f2_DBI_PPI}
    \end{table}
 
   \begin{table}[H]
     \centering
     \begin{tabular}{ c| c c  c  c c  c  c c}
       \hline
       $N_{i}$   & PCHIP     & Rate    && DBI       & Rate    && PPI      & Rate  \\
       \hline
        $17 $	 & 2.42E-2 	 & -- 	 && 2.58E-2 	 & -- 	 && 3.85E-2 	 & --   \\     
        $33 $	 & 4.64E-3 	 & 2.49	 && 6.05E-3 	 & 2.20	 && 1.52E-2 	 & 1.40 \\     
        $65 $	 & 1.34E-3 	 & 1.83	 && 9.31E-4 	 & 2.76	 && 2.85E-3 	 & 2.47 \\     
        $129$ 	 & 2.41E-4 	 & 2.50	 && 2.12E-4 	 & 2.16	 && 2.13E-4 	 & 3.79 \\     
        $257$ 	 & 3.88E-5 	 & 2.65	 && 1.40E-5 	 & 3.95	 && 1.40E-5 	 & 3.95 \\     
       \hline
     \end{tabular}                                                                                  
     \caption{$L^2$-errors and rates of convergence when using the PCHIP method to approximate the function $f_{2}(x)$.
              $N_{i}$ represents the number of input points used to build the approximation.
              The interval $[-0.2,0.2]$ is divided into $(N_{i}-1) / 3$ elements and $4$ LGL quadrature points are used in each element.}
     \label{tab:f2_PCHIP_LGL}
   \end{table}
   %%
   \begin{table}[H]
      \centering
      \begin{tabular}{ c| c  c   c  c  c}
        \hline
        $N_{i}$     & \multicolumn{2}{c}{DBI} && \multicolumn{2}{c}{PPI}   \\
        \hline
                    & $L^{2}$-error & Rate     && $L^{2}$-error & Rate     \\ 
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{1}$}               \\
        \hline
        $17$        & 1.55E-2 	 & --       && 1.55E-2 	 & --       \\
        $33$        & 6.75E-3 	 & 1.25     && 6.75E-3 	 & 1.25     \\
        $65$        & 2.93E-3 	 & 1.23     && 2.93E-3 	 & 1.23     \\
        $129$       & 7.08E-4 	 & 2.07     && 7.08E-4 	 & 2.07     \\
        $257$       & 1.63E-4 	 & 2.13     && 1.63E-4 	 & 2.13     \\
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{4}$}               \\
        \hline
          $17 $	 & 1.26E-2 	 & -- 	    && 2.15E-2 	 & --    \\  
          $33 $	 & 3.11E-3 	 & 2.10     && 4.69E-3 	 & 2.29  \\  
          $65 $	 & 3.42E-4 	 & 3.26     && 3.72E-4 	 & 3.74  \\  
          $129$	 & 1.55E-5 	 & 4.51     && 1.55E-5 	 & 4.64  \\  
          $257$	 & 6.29E-7 	 & 4.65     && 6.29E-7 	 & 4.65  \\  
                 \hline
                             & \multicolumn{5}{c}{$\mathcal{P}_{8}$}      \\
                 \hline
          $17 $	 & 4.87E-3 	 & --	    && 2.73E-2 	 & --    \\  
          $33 $	 & 8.71E-4 	 & 2.59     && 3.39E-3 	 & 3.14  \\  
          $65 $	 & 7.57E-5 	 & 3.60     && 1.22E-4 	 & 4.90  \\  
          $129$	 & 2.17E-6 	 & 5.19     && 2.17E-6 	 & 5.88  \\  
          $257$	 & 1.95E-8 	 & 6.83     && 1.95E-8 	 & 6.83  \\  
                \hline
                            & \multicolumn{5}{c}{$\mathcal{P}_{16}$}     \\
                \hline
          $17 $	 & 3.77E-2 	 & --	    && 3.71E-2 	 & 0     \\  
          $33 $	 & 2.53E-4 	 & 7.54     && 7.57E-3 	 & 2.39  \\  
          $65 $	 & 1.37E-5 	 & 4.30     && 7.46E-5 	 & 6.81  \\  
          $129$	 & 2.19E-7 	 & 6.04     && 2.19E-7 	 & 8.51  \\  
          $257$	 & 1.56E-10 	 & 10.52    && 1.56E-10	 & 10.52 \\  
        \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the DBI and PPI methods to approximate the function $f_{2}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               $\mathcal{P}_{j}$ represents the use of polynomials of degree $ \leq j$, with $j$ being the target degree for each of interval.
               The interval $[-0.2,0.2]$ is divided into $(N_{i}-1) / j$ elements and $j+1$ LGL quadrature points are used in each element.}
      \label{tab:f2_DBI_PPI_LGL}
    \end{table}
 
  \subsection{2D Example: Runge Function}
  \label{subsec:2d_runge}
    This example uses an extended version of the 1D Runge function defined in equation \ref{eq:runeg}.
    \begin{equation}
      f_{7}(x, y) = \frac{1}{1+25(x^2+y^2)}, \quad x\in [-1,1].
    \end{equation}

   \begin{table}[H]
      \centering
      \begin{tabular}{ c| c  c   c  c  c}
        \hline
        $N_{i}$     & \multicolumn{2}{c}{DBI} && \multicolumn{2}{c}{PPI}   \\
        \hline
                    & $L^{2}$-error & Rate     && $L^{2}$-error & Rate     \\ 
        \hline
                    & \multicolumn{5}{c}{$\mathcal{P}_{1}$}               \\
        \hline
 
        \hline
      \end{tabular}                                                                                  
      \caption{$L^2$-errors and rates of convergence when using the DBI and PPI methods to approximate the function $f_{7}(x)$.
               $N_{i}$ represents the number of input points used to build the approximation.
               $\mathcal{P}_{j}$ represents the use of polynomials of degree $ \leq j$, with $j$ being the target degree for each of interval.
               The interval $[-1.0,1.0]$ is divided into $(N_{i}-1) / j$ elements and $j+1$ uniform points are used in each element.}
      \label{tab:f7_DBI_PPI}
    \end{table}

 
  \subsection{2D Example: Smoothed Heaviside Function}
  \label{subsec:2d_example}
    This example uses an extension of the 1D approximation of the Heaviside function $f_{2}(x)$ defined in Equation \ref{eq:f2}.
    The extended version is defined as follows:
    \begin{equation}\label{eq:Heaviside2}
      f_{10}(x,y) = \frac{1}{1+e^{-\sqrt{2}k(x+y)}}, \quad k=100 \textrm{, and } x, y \in [-0.2, 0.2]
    \end{equation}
    The function $f_{10}(x,y)$ is challenging because of the large gradient at $y=-x$.
 

 ------- Function fun = 1  -------- 
 ---- Polynomial degree d = 4  ---- 
17 	 6.643877e-03 	 0 	 5.074580e-03 	 0 	 4.275398e-03 	 0 	 1.245417e-02 	 0 	 5.586907e-03 	 0 	 5.333451e-03 	 0 
33 	 2.342822e-03 	 1.571459e+00 	 3.708873e-04 	 3.944103e+00 	 3.310149e-04 	 3.857216e+00 	 2.810251e-03 	 2.244527e+00 	 4.597794e-04 	 3.765198e+00 	 4.532685e-04 	 3.716705e+00 
65 	 4.686437e-04 	 2.373974e+00 	 2.618011e-05 	 3.910573e+00 	 1.308383e-05 	 4.766017e+00 	 4.454216e-04 	 2.717308e+00 	 2.666875e-05 	 4.200235e+00 	 2.539137e-05 	 4.251603e+00 
129 	 8.657337e-05 	 2.463946e+00 	 1.234794e-06 	 4.455768e+00 	 4.361511e-07 	 4.962094e+00 	 8.941995e-05 	 2.342601e+00 	 7.990353e-07 	 5.117762e+00 	 6.863795e-07 	 5.267875e+00 
257 	 1.565250e-05 	 2.481433e+00 	 5.129779e-08 	 4.615087e+00 	 1.386069e-08 	 5.003791e+00 	 2.011276e-05 	 2.164614e+00 	 2.787254e-08 	 4.868620e+00 	 2.148170e-08 	 5.025985e+00 
 ---- Polynomial degree d = 8  ---- 
17 	 5.009226e-03 	 0 	 3.235526e-03 	 0 	 1.946333e-03 	 0 	 3.258772e-03 	 0 	 3.556469e-03 	 0 	 3.595635e-03 	 0 
33 	 1.226700e-03 	 2.121160e+00 	 2.882368e-04 	 3.645689e+00 	 7.855950e-05 	 4.839250e+00 	 8.584399e-04 	 2.011157e+00 	 9.388677e-05 	 5.479369e+00 	 9.343052e-05 	 5.503226e+00 
65 	 2.334265e-04 	 2.447656e+00 	 2.350478e-05 	 3.697674e+00 	 5.141425e-07 	 7.418884e+00 	 1.876534e-04 	 2.243053e+00 	 1.804951e-06 	 5.829288e+00 	 1.511194e-06 	 6.084145e+00 
129 	 4.265033e-05 	 2.479968e+00 	 1.160491e-06 	 4.389043e+00 	 1.489405e-09 	 8.526276e+00 	 3.749224e-05 	 2.349582e+00 	 4.426131e-08 	 5.410040e+00 	 4.531841e-09 	 8.475801e+00 
257 	 7.721456e-06 	 2.479504e+00 	 4.943028e-08 	 4.578851e+00 	 3.245982e-12 	 8.891683e+00 	 7.318766e-06 	 2.370199e+00 	 1.727347e-09 	 4.705782e+00 	 1.872166e-11 	 7.963864e+00 
 ---- Polynomial degree d = 16  ---- 
17 	 5.009226e-03 	 0 	 3.685871e-03 	 0 	 9.373292e-02 	 0 	 6.311475e-03 	 0 	 7.438853e-03 	 0 	 1.468661e-02 	 0 
33 	 1.226700e-03 	 2.121160e+00 	 2.851465e-04 	 3.858407e+00 	 2.676037e-05 	 1.230417e+01 	 4.153918e-04 	 4.102105e+00 	 2.926470e-05 	 8.349372e+00 	 2.914921e-05 	 9.380850e+00 
65 	 2.334265e-04 	 2.447656e+00 	 2.346475e-05 	 3.684287e+00 	 2.625300e-08 	 1.021848e+01 	 1.072140e-04 	 1.997987e+00 	 8.119699e-07 	 5.288068e+00 	 5.409170e-08 	 9.278198e+00 
129 	 4.265033e-05 	 2.479968e+00 	 1.163450e-06 	 4.382842e+00 	 1.772279e-12 	 1.401068e+01 	 2.464904e-05 	 2.144785e+00 	 2.274240e-08 	 5.216080e+00 	 1.968086e-11 	 1.155311e+01 
257 	 7.721456e-06 	 2.479504e+00 	 4.941608e-08 	 4.582962e+00 	 1.888964e-15 	 9.929426e+00 	 5.197421e-06 	 2.258316e+00 	 9.214896e-10 	 4.651333e+00 	 7.988569e-15 	 1.133005e+01 
 ------- Function fun = 4  -------- 
 ---- Polynomial degree d = 4  ---- 
17 	 1.449656e-02 	 0 	 9.445936e-03 	 0 	 9.639048e-03 	 0 	 1.595854e-02 	 0 	 1.118209e-02 	 0 	 1.136358e-02 	 0 
33 	 2.903438e-03 	 2.424287e+00 	 1.334633e-03 	 2.950317e+00 	 1.407503e-03 	 2.900681e+00 	 3.670497e-03 	 2.215709e+00 	 1.727110e-03 	 2.816042e+00 	 1.706808e-03 	 2.858142e+00 
65 	 3.598792e-04 	 3.080019e+00 	 9.288349e-05 	 3.931473e+00 	 9.288349e-05 	 4.009895e+00 	 5.677027e-04 	 2.753415e+00 	 1.281209e-04 	 3.837303e+00 	 1.281209e-04 	 3.819860e+00 
129 	 3.990021e-05 	 3.208792e+00 	 3.670627e-06 	 4.713838e+00 	 3.670627e-06 	 4.713838e+00 	 9.721598e-05 	 2.574552e+00 	 5.474090e-06 	 4.599990e+00 	 5.474090e-06 	 4.599990e+00 
257 	 4.668283e-06 	 3.112873e+00 	 1.214016e-07 	 4.945878e+00 	 1.214016e-07 	 4.945878e+00 	 2.018363e-05 	 2.280786e+00 	 1.768100e-07 	 4.980251e+00 	 1.768100e-07 	 4.980251e+00 
 ---- Polynomial degree d = 8  ---- 
17 	 8.070214e-03 	 0 	 8.037904e-03 	 0 	 1.176242e-02 	 0 	 1.225034e-02 	 0 	 1.217342e-02 	 0 	 1.226101e-02 	 0 
33 	 1.260990e-03 	 2.798581e+00 	 1.025173e-03 	 3.104666e+00 	 1.944344e-03 	 2.713705e+00 	 2.513146e-03 	 2.388108e+00 	 1.762680e-03 	 2.913367e+00 	 1.547514e-03 	 3.120447e+00 
65 	 1.440938e-04 	 3.199961e+00 	 4.832234e-05 	 4.506290e+00 	 5.092938e-05 	 5.372988e+00 	 3.372199e-04 	 2.962997e+00 	 4.982589e-05 	 5.260603e+00 	 4.982589e-05 	 5.068555e+00 
129 	 1.625898e-05 	 3.183161e+00 	 2.567281e-07 	 7.641435e+00 	 2.567281e-07 	 7.718097e+00 	 4.190406e-05 	 3.042422e+00 	 4.029221e-07 	 7.028553e+00 	 4.029221e-07 	 7.028553e+00 
257 	 1.943423e-06 	 3.081832e+00 	 5.265760e-10 	 8.979694e+00 	 5.265760e-10 	 8.979694e+00 	 5.964498e-06 	 2.828464e+00 	 1.212878e-09 	 8.423116e+00 	 1.212878e-09 	 8.423116e+00 
 ---- Polynomial degree d = 16  ---- 
17 	 8.070214e-03 	 0 	 7.323491e-03 	 0 	 3.988689e-02 	 0 	 1.316061e-02 	 0 	 1.323507e-02 	 0 	 1.253986e-02 	 0 
33 	 1.260990e-03 	 2.798581e+00 	 1.026219e-03 	 2.962797e+00 	 1.753348e-02 	 1.239172e+00 	 2.747470e-03 	 2.361769e+00 	 1.989607e-03 	 2.856852e+00 	 1.935457e-03 	 2.817104e+00 
65 	 1.440938e-04 	 3.199961e+00 	 2.127692e-04 	 2.321102e+00 	 2.392437e-03 	 2.938279e+00 	 3.565614e-04 	 3.012229e+00 	 3.812587e-05 	 5.834072e+00 	 3.848684e-05 	 5.779466e+00 
129 	 1.625898e-05 	 3.183161e+00 	 1.029376e-06 	 7.778027e+00 	 1.029376e-06 	 1.130848e+01 	 4.092514e-05 	 3.158276e+00 	 6.202157e-08 	 9.368151e+00 	 6.202157e-08 	 9.381899e+00 
257 	 1.943423e-06 	 3.081832e+00 	 4.408511e-11 	 1.459288e+01 	 4.408511e-11 	 1.459288e+01 	 5.037159e-06 	 3.039334e+00 	 6.198416e-12 	 1.336345e+01 	 6.198416e-12 	 1.336345e+01 
>> 





















